Oxygen Metallicity Determinations from Optical Emission Lines in Early-type Galaxies

We measured the oxygen abundances of the warm (T$\sim 10^{4}K$) phase of gas in seven early-type galaxies through long-slit observations. A template spectra was constructed from galaxies void of warm gas and subtracted from the emission-line galaxies, allowing for a clean measurement of the nebular lines. The ratios of the emission lines are consistent with photoionization, which likely originates from the UV flux of post-asymototic giant branch (PAGB) stars. We employ H II region photoionization models to determine a mean oxygen metallicity of $1.01\pm0.50$ solar for the warm interstellar medium (ISM) in this sample. This warm ISM 0.5 to 1.5 solar metallicity is consistent with modern determinations of the metallicity in the hot (T$\sim 10^{6}-10^{7}K$) ISM and the upper range of this warm ISM metallicity is consistent with stellar population metallicity determinations. A solar metallicity of the warm ISM favors an internal origin for the warm ISM such as AGB mass loss within the galaxy.

==> f4.tex <==
\begin{figure}
\epsscale{0.75}
\plotone{f4.eps}
\caption[Excitation Diagnostic Diagram]
{Excitation Diagnostic Diagram.  Galaxy line ratios are plotted as filled circles (Table \ref{Xmetal Line Ratios}). 
Excitation diagnostic figure reproduced from \citet{Shock_Photo_1}
(For a full description of this diagnostic diagram see this source). 
Photoionization models from \citet{Photo_3} and 
\citet{Photo_1,Photo_2} trace out the '7' shaped 
tracks and are in good agreement with the data.  The shock 
and shock plus precursor models \citep{Shock_1} 
trace out box shaped regions
in the middle of the plot.  In regions of overlap of the photoionization
regions and shock excitation, the parameters of the model 
(velocities $>$ 350 km/s and high magnetic fields and densities) 
are not representative of the physical conditions in early-type galaxies.
}
\label{xmetal_excitation_diag}
\end{figure}

